TactStyle: Generating Tactile Textures with Generative AI for Digital Fabrication

Recent work in Generative AI enables the stylization of 3D models based on image prompts. However, these methods do not incorporate tactile information, leading to designs that lack the expected tactile properties. We present TactStyle, a system that allows creators to stylize 3D models with images while incorporating the expected tactile properties. TactStyle accomplishes this using a modified image-generation model fine-tuned to generate heightfields for given surface textures. By optimizing 3D model surfaces to embody a generated texture, TactStyle creates models that match the desired style and replicate the tactile experience. We utilize a large-scale dataset of textures to train our texture generation model. In a psychophysical experiment, we evaluate the tactile qualities of a set of 3D-printed original textures and TactStyle's generated textures. Our results show that TactStyle successfully generates a wide range of tactile features from a single image input, enabling a novel approach to haptic design.

==> Sections/12_acknowledgements.tex <==


% \changes{
\begin{acks}
% \section{Acknowledgments}

\changes{
We would like to extend our sincere gratitude to the MIT-Google Program for Computing Innovation for their generous support, which made this research possible. Furthermore, we thank Varun Jampani, Yingtao Tian, Vrushank Phadnis, Yuanzhen Li, and Douglas Eck from Google for their valuable insights and feedback on this research.     
}
\end{acks}

% }

==> Sections/discussion_with_donald.tex <==
Things to do: 
Describe the problems as research questions rather than hypothesis. 
- Are perceptual features from images and tactile surfaces correlated to tactile features in TactStyle? 

- Are perceptual features from images and tactile surfaces correlated to tactile features in Stylization?

- Are the perceptual features from images and tactile surfaces correlated within themselves (our initial assumption) 

Section: 

Results

Subsection: Comparing Perceptual Ratings

Subsection: PErceptual Correlation

Subsection: Mateiral Perception



Discussion section

Mapping Perceptual Features from Images to Tactile

Stylization is significantly bad at (give all the descriptors with the modality)-- Perceptual Ratings 

TactStyle is good at (give all descriptors with the modality) - PErceptual Correlation

Visual and Tactile are correlated at these. 



TactStyle is good at replicating ___ visual features and ___ tactile features. This means a designer can now compose tactile features on a 3D model based on image prompts using cross-modal design approach. Even though that texture might not have the exact tactile features (in the orignal heightmap), visual expectation will match TactStyle's result. 



Figure

Show tactile bar plots with grouped correlation graphs





Tactile features are mapped to visual features - https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=4309999&tag=1

https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8794285

https://www.allpsych.uni-giessen.de/karl/pdf/137.visuohaptic.pdf

https://www.tandfonline.com/doi/pdf/10.1080/10350330.2011.591998

https://www.sciencedirect.com/science/article/pii/S0001691806000382?via%3Dihub

https://www.pnas.org/doi/pdf/10.1073/pnas.1102780108



We have created a pipeline that takes tactile properties from images, and then replicates those features. The result is correlated to the features. 

Stylization is significantly different from visual textures
Stylization is significantly different from original heightfields

Stylization is significantly different from TactStyle

Tactile perception in TactStyle is correlated to perception in visual textures


X. Are we now better than Stylization?
1. Stylization is bad at tactile features -> which features did it do badly?
2. TactStyle is close to the visual -> Which features did it do correclty and which badly? -> where do we need to improve?
3. Visual is close to the original heightmap -> not for everything -> is TactStyle better for some things?

X. Crossmodal design from visual to tactile
- Weirding haptics did audio features to tactile features: \url{https://doi.org/10.1145/3472749.3474797}
- TactStyle does visual features to tactile features
Allows a designer to take a picture of a texture with expected tactile features and then apply those tactile impressions to a 3D print.

% H1: Visual perception is significantly different from tactile sensations
% H1a: Original heightmaps create significantly different sensations than the visual textures
% H1b: Reconstructed samples create significantly different sensations than the visual textures
% H1c: Stylization creates significantly different sensations than the visual textures



==> Sections/implementation.tex <==
\subsection{Simulation Issues}
\textbf{Talk about Semi-Implicit Euler method,} and the requirement to find an efficient delta\_t value. This is important, because too small a value will lead to a very slow simulation, and too large a value will lead to numerical instability. This value changes because stylized models have different geometry, and hence a different delta\_t for their analysis. Before running all the simulations for this, we run binary search for sim\_dt values over a range of values to search for an efficient number that creates a stable simulation, and run that. 

\textbf{Tetrahedralization}: Requires a fast, and efficient method, maximizing the quality while reducing the impact on the speed. 

\textbf{Matching vertices between tetrahedral file and the original mesh:} The OBJ and TET file are different because TET is a volumetric file. We match the vertex by finding an intersection of points from the TET file to the OBJ file, and then propagate the gradients accordingly. 

\subsection{Simulation Issues}
\textbf{Talk about Semi-Implicit Euler method,} and the requirement to find an efficient delta\_t value. This is important, because too small a value will lead to a very slow simulation, and too large a value will lead to numerical instability. This value changes because stylized models have different geometry, and hence a different delta\_t for their analysis. Before running all the simulations for this, we run binary search for sim\_dt values over a range of values to search for an efficient number that creates a stable simulation, and run that. 

\textbf{Tetrahedralization}: Requires a fast, and efficient method, maximizing the quality while reducing the impact on the speed. 

\textbf{Matching vertices between tetrahedral file and the original mesh:} The OBJ and TET file are different because TET is a volumetric file. We match the vertex by finding an intersection of points from the TET file to the OBJ file, and then propagate the gradients accordingly. 



==> Sections/notes.tex <==
ection{What are we doing here?}
For Style2Fab, we manipulated an existing 3D model to ascribe to a particular aesthetic style of the user. Since a 3D model can have multiple functional and aesthetic segments, we first segment the model and preserve the geometric aspects of this model to preserve the overall intended functionality. 

However, we realized that when we manipulate the geometry of the 3D model to get the intended texture of the user, we also affect the physical characteristics of the 3D model. For example, when we manipulated the texture of the splint design to have a blue-kintted texture, we got the desired rough texture, but we also made the model significantly weaker. This leads to the question: Can we use this technique to extend the user's control for physical properties as well? 

Few ideas for the interaction: 

Instead of finding a global level of physical capability (how strong, flexible a model is), we can keep the results relative to the original model. So, when the user first applies the texture to a 3D model, the system will annotate the 3D model to not just show the color and texture, but also give relative strength properties. For example, when the splint design would be highlighted, it will show that the stress / displacement thresholds are 40\% of the original design. Next, the user can use the slider for different properties to control -  for example flexibility, strength etc.  This control can be on the segment level, as well as entire 3D model level. This would require a multi-goal optimization, meaning there will be 2 networks: the Text2Mesh network that manipulates the 3D model for a specific texture, the new property control network that analyzes the physical properties and gives a heatmap. We combine the gradient and send back the results to the interface.  

- Another possible method is to allow a Pareto-Optimal space exploration. Since the stylization and FEA results might have different directional gradients, we can sample that space, and show multiple results that work for a user. Using the thumb splint as an example again: the system could show multiple results: 1) best combination of texture + rigidity 2) flexible 3) flexible on the hand segment + texture 4) best flexibility 5) best texture. The user can now either use one of these results directly, or use one of them as intermediate results, and fine-tune. 

\section{Questions}
\begin{enumerate}
    \item Are we manipulating the model's geometry, or are we changing the 3D printing material to be used for that part? 
    Both approaches have pros and cons. The pros of this approach is that it gives us a good story with the aesthetical property being changed with Style2Fab, and then we have the functional property being manipulated with the geometry as well. The con maybe that the ranges allowed would be limited by the material used. The way we can control this is that we can have an ML network recommend the material to use given the stress and strain regions of the model. This would work well with the J55 printer as well. 

    \item Where are getting the data from ? 
    Design and fabrication of materials with desired deformation behavior (https://dl.acm.org/doi/10.1145/1833349.1778800). This paper talks about collection of a dataset of deformation of 3D printed objects, and then using it as a library to combine internal structures of the model giving certain flexibility properties. 

    \item What are the different properties that we let the user control? 

    \item Can the system give recommendations on printing a model with specific materials as well, given the FEA results ? For example, a 3D model that has high displacement values, and low stress thresholds should be printed with certain flexible materials. 

\end{enumerate}
    



Useful phrases: 
As humans, we regularly link shape of an object with its built material. But in the context of geometric modeling, this inter-relation between form and material is rarely explored. 

\subsection{Experiments}
\paragraph{How much does the FEA result change when we use Text2Mesh on a model? Does it vary across prompts?:}

We sample 100 3D models from a Thingiverse dataset, and stylize them. We get the FEA analysis done both before and after stylization. We applied a variety of different textures: \faraz{What are these textures?} We found that the on average, XX property changed by YY, \faraz{Make a table. }

This means the following. 

\paragraph{Can we use FEA results as gradients to improve specific physical properties?: }

\paragraph{Can the FEA results be used in combination with the gradients from Text2Mesh?: }

\paragraph{Can we create a Pareto Optimal Space here, and sample points here to get models with those properties?: }

Amira: This is a question that people are still exploring. There are multiple approaches for it - for example: controlling the global properties by making local changes. 
Two approaches: Morphing the geometry

\paragraph{How do we define flexibility, and these properties? }
Flexibility == compliance. 
Maximum compliance doesn't make sense. 
If we keep the volume of the material between the models to be the same, then we can compare the compliance. 

There are ways to keep the same volume but increase or decrease the compliance. 

The model needs to be remeshed to have tetrahedrals instead of the tri-meshes. 

Get gradSim to work on a machine and let Amira know. Try out gradSim as a replacement for FEA. Think about an argument why it would make sense to have that instead of FEA, or maybe some combination. 
Particle systems are easier to simulate. 


==> Sections/perception_copy.tex <==
\section{Perception Study}
In order to evaluate TactStyle's accuracy at replicating the tactile feedback of textures, we performed a blind-perception user study, which is a psycho-physical experiment used to evaluate texture replication techniques~\cite{degraen2021capturing, perez2016optimization}. The goal of our study was to understand if the reconstructed heighfield from TactStyle creates similar tactile perceptions to the original heightfield. In addition, our second goal was to evaluate if the tactile perception of TactStyle's heightfield are similar to the expected tactile perception from just looking at a visual image of the texture. 

% TactStyle is a system that takes a texture image and generates a heightfield that can be applied to a 3D model during stylization. This heightfield generation technique assumes a correlation between the visual properties of a texture, and their tactile properties, which TactStyle approximates using the fine-tuned image-generation model. 

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/evaluation-models.png}
    % \vspace{-3mm}
    \caption{3D-Printed samples of 15 textures from our test set used in perception study: We created four different sets for our perception study: the `visual set', `original set', `reconstructed set', and the `baseline set'. The original set was created with the height associated to the texture and served as the groundtruth. The reconstructed set was created using TactStyle, with the texture image as input. The visual set was created using printed texture images. Finally, the baseline set was created using Style2Fab, using the texture as input. }
    % \vspace{-5mm}
    \label{fig:study_models}
\end{figure*}



\subsection{Conditions}
We created four different conditions as shown below:

\begin{enumerate}
    \item \textbf{Visual (No Heightfield):} The texture image was printed with no heightfield on glossy paper and pasted on flat tiles. 
    \item \textbf{Original Heighfield:} The tile contained the heightfield originally provided with the texture (groundtruth).
    \item \textbf{TactStyle:} The `TactStyle' set was created using our system with the texture image as input.
    \item \textbf{Stylization Only:} Finally, the `Stylization only' set was created using Style2Fab, using the texture image as input, resulting in a heightfield that best approximates the visual style but does not consider tactile properties.
\end{enumerate}

\subsection{Hypothesis}

In this experiment, we evaluate the following: 
\begin{enumerate}
   \item \textbf{Hypothesis 1 (Touching):} There is a similarity in the tactile properties `perceived' by touching the original texture (original condition) and the tactile properties `perceived' by touching the replicated texture (TactStyle condition), but not between the original texture (original condition) and the replicated texture (Stylization only condition).

    \item \textbf{Hypothesis 2 (Touching vs. Vision):} There is a similarity in the tactile properties `perceived' by touching both the original and the TactStyle texture and the tactile properties `expected' by looking at the texture (visual condition), but not between the stylized-only texture and the visual texture.
    
\end{enumerate}

% \begin{enumerate}
%    \item \textbf{Hypothesis 1 (Original vs. TactStyle)):} There is a similarity in the tactile properties `perceived' by touching the original texture (original condition) and the tactile properties `perceived' by touching the replicated texture (TactStyle condition).

%     \item \textbf{Hypothesis 2 (Original vs. Stylization-Only):} There is no similarity in the tactile properties `perceived' by touching the original texture (original condition) and the tactile properties `perceived' by touching the 
%      replicated texture (Stylization only condition).

%     \item \textbf{Hypothesis 3 (Original vs. Visual):} There is a similarity in the tactile properties `perceived' by touching the texture (original condition) and the tactile properties `expected' by looking at the texture (visual condition).

%     \item \textbf{Hypothesis 4 (TactStyle vs. Visual):} There is a similarity in the tactile properties `perceived' by touching the replicated texture (TactStyle condition) and the tactile properties `expected' by looking at the texture (visual condition).
    
%     \item \textbf{Hypothesis 5 (Stylization-only vs. Visual):} There is a similarity in the tactile properties `perceived' by touching the replicated texture (Stylization only condition) and the tactile properties  `expected' by looking at the texture (visual condition).

% \end{enumerate}

\subsection{Dataset}
We collected 15 random samples from our test set, matching the size of the sample set used by Degraen et al.~\cite{degraen2021capturing} in their study on the perceptual similarity between real textures and their digital replicas. As these textures were not used to train the model, they can be used to evaluate TactStyle's ability to replicate unseen textures. Figure~\ref{fig:study_models} shows the models used in our study. This gave us a total set of 60 models (4 conditions for each of the 15 textures). All the conditions were presented to the user on tiles of the same size - 5cm x 5cm x 1cm.



\subsection{Study Design}
% We collected 15 random samples from our test set, matching the size of the sample set used by Degrean et al.~\cite{degraen2021capturing} in their study. 
We used a within-subjects experimental design. To counter-balance carry-over effects, \stefanie{we used a round-robin ordering of the sample sets} between participants. During the study, each participant recorded their ratings of the sample in terms of hardness, roughness, bumpiness, stickiness, scratchiness, uniformity, and \stefanie{degree of uniformity}, each on a 1-to-9 Likert scale. A value of 1 indicated a low \stefanie{assessment}, and 9 indicated a high assessment. These descriptors were drawn from Degraen et al.~\cite{degraen2021capturing}. We use all the descriptors from this prior study except for `hairiness', since none of the textures in our dataset were representative of `hairy' textures. 

Our study was structured as a self-assessment test in which participants compare and record the perceptual attributes of these 3D-printed texture samples.

The experimenter noted the response for each trial and placed the next sample. \stefanie{The participant was asked the following questions for each sample}: 
\begin{enumerate}
    \item[Q1:] How \textbf{hard} does this surface feel? (1 meaning extremely soft, 9 meaning extremely hard)

    \item[Q2:] How \textbf{rough} does this surface feel? (1 meaning extremely smooth, 9 meaning extremely rough)

    \item[Q3:] How \textbf{bumpy} does this surface feel? (1 meaning extremely fat, 9 meaning extremely bumpy)

    \item[Q4:] How \textbf{sticky} does this surface feel? (1 meaning extremely slippery, 9 meaning extremely sticky)

    \item[Q5:] How \textbf{scratchy} does this surface feel? (1 meaning extremely dull, 9 meaning extremely scratchy)

    \item[Q6:] How \textbf{uniform} does this surface feel? (1 meaning extremely irregular, 9 meaning extremely uniform)

    \item[Q7:] How \textbf{isotropic} \stefanie{does this surface feel}? (1 meaning extremely anisotropic, 9 meaning extremely isotropic)
    
    % \item[Q8:] What kind of material is this? (Open question)
\end{enumerate}


\subsection{Apparatus}
Our apparatus was built to limit visual cues and ensure accurate recording of purely tactile perceptual attributes of the textures. Participants were positioned in front of a screen that separated them from the experimenter, as shown in Figure~\ref{fig:study_setup}. A small opening in the screen, covered by a piece of cloth, allowed participants to reach through and access the samples, placed by the experimenter. On the other side, the experimenter arranged the samples for the participants to explore. The samples were held in place with a laser-cut wooden frame. The order in which the samples were presented was \stefanie{organized in a spreadsheet, where the experimenter also recorded the participants' responses}.

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/study_setup.png}
    % \vspace{-3mm}
    \caption{Experimental Setup for perception study: a) Experimenter side, b) Participant side}
    % \vspace{-5mm}
    \label{fig:study_setup}
\end{figure*}



\subsection{Participants}
A total of 15 participants (6 female, 9 male, 22 - 38 years, $M=27.3$ years, $SD=5.4$) with backgrounds in \stefanie{Design, Electrical Engineering, Computer Science, Material Science, Aeronautics, Architecture, and Political Science} were recruited for our study. When asked about their hand dominance, 14 participants indicated to be right-handed with 1 participant indicating ambidexterity. All participants chose to use their right-hand index finger. They were informed that they could only use this finger throughout the study. All participants indicated that they do not suffer from any impairment to haptic perception to best of their knowledge. Participants were compensated with \$40 an hour for the 90-minutes long study.
% When asked about how often they performed



\subsection{Study Procedure}
The total study duration was set to be 90 minutes. At the start, participants were asked to fill in a short survey about their demographic data. Next, to ensure that participants clearly understood the perceptual descriptors used in the study, we conducted a short training session where participants were allowed to explore exemplar structures separate from the set being investigated. Once they were confident in their understanding of the descriptors, we proceeded to the evaluation stage. 

%We use the same descriptors. \faraz{cite the section where you introduced this concept.} 
 
During this stage, the experimenter placed one sample at a time on a fixed location behind a screen. The participant could insert their hand into the curtain and feel the texture but were not allowed to see the texture itself. The participant was then asked to explore the texture and rate its tactile properties based on the 7 descriptors. 

 \subsection{Results}

 \begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Perception_Graphs_comparing_types.png}
    % \vspace{-3mm}
    \caption{Box Plots showing the individual assessments on Hardness, Roughness, Bumpiness, Stickiness, Scratchiness, Uniformity, and Isotropy}
    % \vspace{-5mm}
    \label{fig:study_models}
\end{figure*}

 \begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Correlations.png}
    % \vspace{-3mm}
    \caption{Box Plots showing the individual assessments on Hardness, Roughness, Bumpiness, Stickiness, Scratchiness, uniformity, and Isotropy}
    % \vspace{-5mm}
    \label{fig:study_models}
\end{figure*}


In this section, we detail the analysis of the results from the perception study. Our goal was to evaluate if TactStyle is effective in replicating the tactile feedback of textures and performs better than current stylization methods. We analyze and report results for each descriptor individually. To analyze the individual tactile assessments, we conducted Friedman tests with post-hoc analysis using Wilcoxon signed-ranks tests.


\subsubsection{Bumpiness}
% Friedman test statistic: 95.71578947368414
% P-value: 1.2956286185355336e-20\

The ratings of bumpiness were found to significantly differ depending on the presented texture (${\chi}^2(3) = 95.716$, $p < .001$).

\textbf{Hypothesis 1 (Touching)}:  The TactStyle samples were significantly higher in bumpiness ratings compared to the original samples ($W = 6257.5$, $p < .01$)


\textbf{Hypothesis 2 (Visual)}: 



The stylization samples were perceived to be significantly higher in terms of bumpiness compared to the visual textures ($W = 3901.5$, $p < .001$), the original samples ($W = 2296.0$, $p < .001$) and the reconstructed samples ($W = 3326.0$, $p < .001$).


, but no significant differences were found for bumpiness ratings between the visual textures and the original samples ($W = 7070.0$, $p = .236$) and the reconstructed samples ($W = 8242.54$, $p = .236$).

Our results reveal that stylization generated samples with significantly higher bumpiness perception, while our reconstruction approach provided sensations closer to the visual textures than the original samples.

% \begin{itemize}
%     \item \textit{Image / Original}: W = 7070.0, p = 0.236
%     \item \textit{Image / Reconstructed}: W = 8242.54, p = 0.236
%     *\item \textit{Image / Stylized}: W = 3901.5, p < 0.001 ***
%     \item \textit{Original / Reconstructed}: W = 6257.5, p < 0.01 **
%     *\item \textit{Original / Stylized}: W = 2296.0, p < 0.001 ***
%     *\item \textit{Reconstructed / Stylized}: W = 3326.0, p < 0.001 ***
% \end{itemize}

%   Surface_Type  min  max       std  median      mean
% 0            I    1    9  2.463882       3  4.026667
% 1            O    1    9  2.164083       3  3.702222
% 2            R    1    9  1.978736       4  4.297778
% 3            S    1    9  2.235465       6  5.804444

% Wilcoxon Test Statistics Matrix:

% Image / Original = 7070.0
% Image / Reconstructed = 8242.54
% Image / Stylized = 3901.5
% Original / Reconstructed = 6257.5
% Original / Stylized = 2296.0
% Reconstructed / Stylized = 3326.0

% Corrected P-Values Matrix (Bonferroni-Holm):

% Image / Original = 2.36e-1
% Image / Reconstructed = 2.36e-1
% Image / Stylized = 2.65e-12
% Original / Reconstructed = 3.56e-3
% Original / Stylized = 5.42e-18
% Reconstructed / Stylized = 1.79e-12


\subsubsection{Hardness}
% Friedman test statistic: 29.39772727272689
% P-value: 1.8473340118509612e-06
The ratings of hardness were found to significantly differ depending on the presented texture (${\chi}^2(3) = 29.398$, $p < .001$).
Pairwise analysis revealed a significant decrease in perceived hardness between the visual textures and the original samples ($W = 2476.5$, $p < .001$), the reconstructed samples ($W = 2978.5$, $p < .001$), and the stylized samples ($W = 4319.5$, $p < .001$).
Similarly, the stylized samples were significantly lower in hardness perception than the original samples ($W = 1161.5$, $p < .01$) and the reconstructed samples ($W = 1080.5$, $p < .001$).

\stefanie{These results reveal our reconstruction method generated samples that were closer in tactile hardness to the samples created from the original heightfields.}
On the other hand, \stefanie{stylization} generated samples that provided hardness sensations in between the visual textures and their original heightfields.

% \begin{itemize}
%     \item \textit{Image / Original}: W = 2476.5, p < 0.001 ***
%     \item \textit{Image / Reconstructed}: W = 2978.5, p < 0.001 ***
%     \item \textit{Image / Stylized}: W = 4319.5, p < 0.001 ***
%     \item \textit{Original / Reconstructed}: W = 927.5, p = 0.17
%     \item \textit{Original / Stylized}: W = 1161.5, p < 0.01 **
%     \item \textit{Reconstructed / Stylized}: W = 1080.5, p < 0.001 ***
% \end{itemize}

%   Surface_Type  min  max       std  median      mean
% 0            I    1    9  2.129135       7  6.773333
% 1            O    4    9  0.978175       8  7.782222
% 2            R    3    9  1.026088       8  7.693333
% 3            S    2    9  1.395031       7  7.462222

% between the image and the original ($W = 2476.5, p < .001$)

% Wilcoxon Test Statistics 
% Image / Original = 2476.5
% Image / Reconstructed = 2978.5
% Image / Stylized = 4319.5
% Original / Reconstructed = 927.5
% Original / Stylized = 1161.5
% Reconstructed / Stylized = 1080.5

% Corrected P-Values Matrix (Bonferroni-Holm):
% Image / Original = 4.2e-9
% Image / Reconstructed = 2.0e-7
% Image / Stylized = 0.00065
% Original / Reconstructed = 1.7e-1
% Original / Stylized = 0.00312
% Reconstructed / Stylized = 1.79e-12

\subsubsection{Roughness}
% Friedman test statistic: 46.48187311178224
% P-value: 4.4795076769122596e-10

\textbf{Hypothesis 1 (Touching)}: The ratings of roughness were found to significantly differ depending on the presented texture (${\chi}^2(3) = 46.482$, $p < .001$).

The roughness perceived in the TactStyle condition was significantly higher than the original condition. i.e., Hypothesis 3 is False. Finally, the roughness perceived in the 'Stylization only' condition was significantly higher than both Visual condition, and the Original condition, i.e, both Hypothesis 4 and 5 are False.   


The samples from the `original' condition were perceived significantly lower in terms of roughness than the `visual' condition ($W = 5768.0$, $p < .001$) and the \stefanie{TactStyle condition} ($W = 4511.0$, $p < .001$). The `Stylization only' condition provided a significantly higher sensation of roughness than the `visual condition' ($W = 6526.0$, $p < .01$), and the `original condition' ($W = 4347.5$, $p < .001$) 
% and the reconstructed samples ($W = 7110.0$, $p < .01$).
\stefanie{No significant difference of roughness perception was found between the visual textures and the reconstructed samples} ($W = 8503.0$, $p = .696$). 
These results indicate that the original set provided a significantly lower roughness sensation compared to that of the visual set, i.e., Hypothesis 1 is False. 

However, the TactStyle condition did provide roughness sensation similar to that of the visual set i.e., Hypothesis 2 is True.


\stefanie{These results indicate that TactStyle provided roughness impressions that were closely related to the visual appearance.
While the `Original' set provided lower sensations of hardness,  and the `Stylization' set significantly increased hardness overall.}

% \begin{itemize}
%     \item \textit{Image / Original}: W = 5768.0, p < 0.001 ***
%     \item \textit{Image / Reconstructed}: W = 8503.0, p = 0.696
%     \item \textit{Image / Stylized}: W = 6526.0, p < 0.01 **
%     \item \textit{Original / Reconstructed}: W = 4511.0, p < 0.001 ***
%     \item \textit{Original / Stylized}: W = 4347.5, p < 0.001 ***
%     \item \textit{Reconstructed / Stylized}: W = 7110.0, p < 0.01 **
% \end{itemize}


%   Surface_Type  min  max       std  median      mean
% 0            I  1.0  9.0  2.142466     4.0  4.595556
% 1            O  1.0  8.0  1.837387     3.0  3.911111
% 2            R  1.0  9.0  1.596959     5.0  4.648889
% 3            S  1.0  9.0  2.097447     6.0  5.226667

% Wilcoxon Test Statistics Matrix:

% Image / Original = 5768.0
% Image / Reconstructed = 8503.0
% Image / Stylized = 6526.0
% Original / Reconstructed = 4511.0
% Original / Stylized = 4347.5
% Reconstructed / Stylized = 7110.0

% Corrected P-Values Matrix (Bonferroni-Holm):

% Image / Original = 7.8e-4
% Image / Reconstructed = 0.696
% Image / Stylized = 6.05e-3
% Original / Reconstructed = 0.000003
% Original / Stylized = 8.610169e-10
% Reconstructed / Stylized = 5.374563e-3


\subsubsection{Scratchiness}
% Friedman test statistic: 45.206072672971665
% P-value: 8.365102819243038e-10

\textbf{Hypothesis 1 (Touching)}: 

\textbf{Hypothesis 2 (Visual)}: 
The ratings of scratchiness were found to significantly differ depending on the presented texture (${\chi}^2(3) = 45.206$, $p < .001$).
The stylized samples were perceived to be significantly higher in terms of scratchiness perception than the visual textures, the original samples and the reconstructed samples.
The ratings for scratchiness for the visual textures were significantly higher than the ratings for the original samples ($W = 6383.5$, $p < .001$) and the reconstructed samples ($W = 6379$, $p < .01$).
No significant difference was found between the scratchiness perception of the original samples and the reconstructed samples ($W = 6907.0$, $p = .410$).

From our results, we see that stylization significantly increased scratchiness ratings, while our reconstruction process generated samples found to be perceptually closer to the original samples compared to the visual textures.


% \begin{itemize}
%     \item \textit{Image / Original}: W = 6383.5, p < 0.001 ***
%     \item \textit{Image / Reconstructed}: W = 6379, p < 0.01 **
%     *\item \textit{Image / Stylized}: W = 8198.0, p < 0.05 *
%     \item \textit{Original / Reconstructed}: W = 6907.0, p = 0.410
%     *\item \textit{Original / Stylized}: W = 4940.5, p < 0.001 ***
%     *\item \textit{Reconstructed / Stylized}: W = 4379.0, p < 0.001 ***
% \end{itemize}


%   Surface_Type  min  max       std  median      mean
% 0            I    1    9  2.252362       5  4.631111
% 1            O    1    9  1.934185       4  3.933333
% 2            R    1    9  1.790329       4  4.008889
% 3            S    1    9  2.155677       6  5.164444


% Wilcoxon Test Statistics Matrix:

% Image / Original = 6383.5
% Image / Reconstructed = 6379
% Image / Stylized = 8198.0
% Original / Reconstructed = 6907.0
% Original / Stylized = 4940.5
% Reconstructed / Stylized = 4379.0

% Corrected P-Values Matrix (Bonferroni-Holm):

% Image / Original = 4.6e-4
% Image / Reconstructed = 3.2e-3
% Image / Stylized = 3.5e-2
% Original / Reconstructed = 4.1e-1
% Original / Stylized = 2.1e-8
% Reconstructed / Stylized = 1.08e-9


\subsubsection{Stickiness}
% Friedman test statistic: 24.53619153674846
% P-value: 1.930206918774562e-05
The ratings of stickiness were found to significantly differ depending on the presented texture (${\chi}^2(3) = 24.536$, $p < .001$).
The stylized samples were found to be significantly higher in stickiness ratings compared to the visual textures ($W = 5679.0$, $p < .01$) and the original samples ($W = 3685.5$, $p < .001$).
The reconstructed samples were found to be significantly higher in stickiness ratings compared to the original samples ($W = 3726.0$, $p < .01$).
No differences were found between the visual textures and the original samples ($W = 5656.5$, $p = 0.085$), and the reconstructed samples ($W = 6985.0$, $p = 0.33$), and between the reconstructed samples and the stylized samples ($W = 5316.0$, $p = .085$).

From our results, we note that stylization significantly increased stickiness, while the reconstruction process created stickiness ratings closer to the visual textures than to the original heightfield.

% \begin{itemize}
%     \item \textit{Image / Original}: W = 5656.5, p = 0.085
%     \item \textit{Image / Reconstructed}: W = 6985.0, p = 0.33
%     \item \textit{Image / Stylized}: W = 5679.0, p < 0.01 **
%     \item \textit{Original / Reconstructed}: W = 3726.0, p < 0.01 **
%     \item \textit{Original / Stylized}: W = 3685.5, p < 0.001 ***
%     \item \textit{Reconstructed / Stylized}: W = 5316.0, p = 0.085
% \end{itemize}

%   Surface_Type  min  max       std  median      mean
% 0            I    1    8  1.840624       4  3.977778
% 1            O    1    8  1.717672       3  3.622222
% 2            R    1    9  1.647509       4  4.133333
% 3            S    1    9  1.957383       4  4.511111

% Wilcoxon Test Statistics Matrix:

% Image / Original = 5656.5
% Image / Reconstructed = 6985.0
% Image / Stylized = 5679.0
% Original / Reconstructed = 3726.0
% Original / Stylized = 3685.5
% Reconstructed / Stylized = 5316.0

% Corrected P-Values Matrix (Bonferroni-Holm):

% Image / Original = 0.085
% Image / Reconstructed = 0.33
% Image / Stylized = 0.009
% Original / Reconstructed = 0.0017
% Original / Stylized = 0.000003
% Reconstructed / Stylized = 0.085

\subsubsection{Uniformity}
% Friedman test statistic: 25.01924050632895
% P-value: 1.529813054350841e-05
The ratings of uniformity were found to significantly differ depending on the presented texture (${\chi}^2(3) = 25.019$, $p < .001$).
Pairwise analysis revealed a significant difference in the ratings of uniformity between the visual textures and the reconstructed samples ($W = 5534.0$, $p < .001$) and the stylized samples ($W = 7579.0$, $p < .05$).
Here, the visual textures were perceived as more uniform than the reconstructed and stylized samples.
No differences were found between the visual textures and the original samples ($W = 7504.0$, $p = .484$), between the original samples and the reconstructed samples ($W = 6783.0$, $p = .115$) and the stylized samples ($W = 7393.5$, $p = .484$), and between the reconstructed and stylized samples ($W = 8565.5$, $p = 0.50$).

These results reveal that our reconstruction process reduced uniformity similarly to the stylization process.


% \begin{itemize}
%     \item \textit{Image / Original}: W = 7504.0, p = 0.484
%     \item \textit{Image / Reconstructed}: W = 5534.0, p < 0.001 ***
%     \item \textit{Image / Stylized}: W = 7579.0, p < 0.05 *
%     \item \textit{Original / Reconstructed}: W = 6783.0, p = 0.115
%     \item \textit{Original / Stylized}: W = 7393.5, p = 0.484
%     \item \textit{Reconstructed / Stylized}: W = 8565.5, p = 0.50
% \end{itemize}


%   Surface_Type  min  max       std  median      mean
% 0            I    1    9  2.263960       7  6.524444
% 1            O    1    9  2.225617       7  6.244444
% 2            R    1    9  2.111599       6  5.808889
% 3            S    1    9  1.870489       7  5.964444

% Wilcoxon Test Statistics Matrix:

% Image / Original = 7504.0
% Image / Reconstructed = 5534.0
% Image / Stylized = 7579.0
% Original / Reconstructed = 6783.0
% Original / Stylized = 7393.5
% Reconstructed / Stylized = 8565.5

% Corrected P-Values Matrix (Bonferroni-Holm):

% Image / Original = 0.484
% Image / Reconstructed = 0.0007
% Image / Stylized = 0.032
% Original / Reconstructed = 0.115
% Original / Stylized = 0.484
% Reconstructed / Stylized = 0.50

\subsubsection{Isotropy}
% Friedman test statistic: 27.13643178410781
% P-value: 5.512084666725917e-06
The ratings of isotropy were found to significantly differ depending on the presented texture (${\chi}^2(3) = 27.136$, $p < .001$).
Pairwise analysis revealed a significant increase in perceived isotropy between the stylized samples and the visual textures ($W = 5726.0$, $p < .001$), the original samples ($W = 6651.5$, $p < .01$), and the reconstructed samples ($W = 5085.5$, $p < .001$).
No significant difference was found for isotropy ratings between the visual textures and the original samples ($W = 7527.5$, $p = .122$), and the reconstructed samples ($W = 7825.0$, $p = .466$), or between the original samples and the reconstructed samples ($W = 7359.5$, $p = .467$).

These results show that the stylization process generated significantly more isotropic samples, while the reconstruction process generated samples closer to the visual textures and original heightfields.

% \begin{itemize}
%     \item \textit{Image / Original}: W = 7527.5, p = 0.122
%     \item \textit{Image / Reconstructed}: W = 7825.0, p = 0.466
%     \item \textit{Image / Stylized}: W = 5726.0, p < 0.001 ***
%     \item \textit{Original / Reconstructed}: W = 7359.5, p = 0.467
%     \item \textit{Original / Stylized}: W = 6651.5, p < 0.01 **
%     \item \textit{Reconstructed / Stylized}: W = 5085.5, p < 0.001 ***
% \end{itemize}


%   Surface_Type  min  max       std  median      mean
% 0            I    1    9  2.489199       4  4.537778
% 1            O    1    9  2.315510       5  4.995556
% 2            R    1    9  2.245427       4  4.804444
% 3            S    1    9  2.047482       6  5.702222

% Wilcoxon Test Statistics Matrix:

% Image / Original = 7527.5
% Image / Reconstructed = 7825.0
% Image / Stylized = 5726.0
% Original / Reconstructed = 7359.5
% Original / Stylized = 6651.5
% Reconstructed / Stylized = 5085.5

% Corrected P-Values Matrix (Bonferroni-Holm):

% Image / Original = 0.122
% Image / Reconstructed = 0.466
% Image / Stylized = 0.000002
% Original / Reconstructed = 0.467
% Original / Stylized = 0.0012
% Reconstructed / Stylized = 0.000023

\subsection{Discussion}



 

 




==> Sections/questions.tex <==
% \section{Questions people might have}
% % \textbf{Why not just track the shell thickness as the stylization is progressing, and stop it where you go too far? }
% % Shell Thickness can be a useful heuristic, but how do you know when a certain part is too thin? Which parts need to be thicker than the rest of parts? Which part the stress will be high, so it should have more material, and so on. 
% % But shell thickness can be used to figure out when to run the simulation! 

% \textbf{Why don't you stylize till the finish, and then get the mask, and re-simulate?} Two ways to argue: we either create such a mask and show that this doesn't give as good results (higher mechanical loss and higher style loss). Or we could report how many models were manipulated beyond repair. 


% \textbf{Why can't you say something is going to break?} This is a low fidelity simulation, where we simulate impulse forces that objects might sustain in real-world usage. In mechanical engineering, different types of materials are simulated under different loading conditions, along with different properties: such as ductility or brittleness of the material. Moreover, the material properties are heavily dependent upon fabrication method, the slicing settings of the model etc. We try to capture some of these properties, by incorporating a material specific properties, and using a PDE based simulation method. But not all properties can be captured by this fast but approximate simulation. However, it informs the stylization about weak sections, and strengthens the local sections to an extent. 

% \textbf{Why can't we just do a post-hoc simulation like Stress Relief or Stochastic Context Aware Analysis and repair the parts that are broken?} Stylization does random changes on the model, and thus can also create visually accurate, but non-printable files with disconnected parts. Repairing those parts will take manual work from the user, or re-stylization with a controlled mask defined for the parts that got broken. This would require a few iterations of identification of weak or missing segments, and correcting the stylization to avoid issues in those local parts. Having an in-situ simulation would detect those segments during the stylization process and update the mask on model, avoiding those issues to occur in a single-run. 

% \textbf{You use a heuristic method to detect when to simulate. Why is that needed and how do you know that's accurate?} Simulation is expensive, and we can't run simulation on every stylization iteration, since that will take a long time to finish the stylization process. Mechnical property change is also a function of the specific model and the stylization prompt, meaning we don't need the same frequency of simulation for different stylizations. Thus, we need a detection method to know when it would be informative to run a simulation to gather data on the mechanical property change in a model. We use the modified shell thickness of the model as a heuristic, since that represents how much material would be at a particular point in the model, and thus have different structural strengths. We don't use the shell thickness to create the mask, since different materials have different properties, and thus would have different responses to the same shell thickness. However, as the shell thickness changes, the mechanical properties change. Knowing this, we use this property to detect when to run a simulation. We show that by using this as a heuristic, we are able to reduce the number of required simulations, while stylizing models in a manner that preserves their mechanical properties from drastically changing. 


